FinGAT: Financial Graph Attention Networks for Recommending Top-K Profitable Stocks

Financial technology (FinTech) has drawn much attention among investors and companies. While conventional stock analysis in FinTech targets at predicting stock prices, less effort is made for profitable stock recommendation. Besides, in existing approaches on modeling time series of stock prices, the relationships among stocks and sectors (i.e., categories of stocks) are either neglected or pre-defined. Ignoring stock relationships will miss the information shared between stocks while using pre-defined relationships cannot depict the latent interactions or influence of stock prices between stocks. In this work, we aim at recommending the top-K profitable stocks in terms of return ratio using time series of stock prices and sector information. We propose a novel deep learning-based model, Financial Graph Attention Networks (FinGAT), to tackle the task under the setting that no pre-defined relationships between stocks are given. The idea of FinGAT is three-fold. First, we devise a hierarchical learning component to learn short-term and long-term sequential patterns from stock time series. Second, a fully-connected graph between stocks and a fully-connected graph between sectors are constructed, along with graph attention networks, to learn the latent interactions among stocks and sectors. Third, a multi-task objective is devised to jointly recommend the profitable stocks and predict the stock movement. Experiments conducted on Taiwan Stock, S&P 500, and NASDAQ datasets exhibit remarkable recommendation performance of our FinGAT, comparing to state-of-the-art methods.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tables/feature.tex <==
\begin{table}[!t]
\caption{feature discription}
\label{tab:feature}
\centering
\begin{tabular}{c|l|cl}
\hline
\multicolumn{2}{c|}{features}                                                                                                   & \multicolumn{2}{c}{calculation}          \\ \hline
\multicolumn{2}{c|}{c\_open, c\_high, c\_low}                                                                                 & \multicolumn{2}{c}{e.g., c\_open = $\frac{open_t}{close_t}-1$}      \\
\multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}5\_days , 10\_days ,\\ 15\_days , 20\_days,\\ 25\_days ,  30\_days\end{tabular}} & \multicolumn{2}{c}{e.g., 5\_days =$\frac{\frac{\sum_{i=0}^4 adj-close_t}{5}}{adj-close_t}-1$}      \\ \hline
\end{tabular}
\end{table}




==> tables/result_50_50.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\centering
\caption{Performance comparison between baselines and the GraphFin with $\mathbf{50\%}$ training $\mathbf{50\%}$ testing}
\label{tab:main_50}
\begin{tabular}{c|cc|cc|cc|l}
\hline
         & \multicolumn{2}{c|}{k = 5} & \multicolumn{2}{c|}{k = 10} & \multicolumn{2}{c|}{k = 20} & \multicolumn{1}{l}{Overall} \\ \cline{2-8} 
Model    & MRR         & Precision    & MRR         & Precision     & MRR         & Precision     & ACC                         \\ \hline
SVR      & 0.2121      & 0.0348       & 0.4405      & 0.0723        & 0.9349      & 0.1732        & 0.4485                      \\
XGBoost  & 0.2910      & 0.0602       & 0.5562      & 0.1204        & 1.0420      & 0.2085        & 0.4293                      \\
MLP      & 0.2687      & 0.0512       & 0.5855      & 0.1123        & 1.1250      & 0.1819        & 0.4477                      \\
GRU      & 0.3432      & 0.0753       & 0.6446      & 0.1228        & 1.1728      & 0.2132        & 0.4874                      \\
GRU+Att  & 0.3798      & 0.0942       & 0.7015      & 0.1359        & 1.2074      & 0.2381        & \multicolumn{1}{c}{0.4905}  \\
Finet    & 0.4009      & 0.1028       & 0.7556      & 0.1492        & 1.2496      & 0.2098        & \multicolumn{1}{c}{0.5124}  \\
GraphFin & 0.4929      & 0.1183       & 0.8321      & 0.1822        & 1.3277      & 0.2600        & \multicolumn{1}{c}{0.5653}  \\ \hline
Improv.  & 22.95\%     & 15.08\%      & 10.12\%     & 22.12\%       & 6.25\%      & 8.42\%        & \multicolumn{1}{c}{10.32\%} \\ \hline
\end{tabular}
\end{table}

